Refinements for Multiparty Message-Passing Protocols: Specification-agnostic theory and implementation

Multiparty message-passing protocols are notoriously difficult to design, due to interaction mismatches that lead to errors such as deadlocks. Existing protocol specification formats have been developed to prevent such errors (e.g. multiparty session types (MPST)). In order to further constrain protocols, specifications can be extended with refinements, i.e. logical predicates to control the behaviour of the protocol based on previous values exchanged. Unfortunately, existing refinement theories and implementations are tightly coupled with specification formats. This paper proposes a framework for multiparty message-passing protocols with refinements and its implementation in Rust. Our work decouples correctness of refinements from the underlying model of computation, which results in a specification-agnostic framework. Our contributions are threefold. First, we introduce a trace system which characterises valid refined traces, i.e. a sequence of sending and receiving actions correct with respect to refinements. Second, we give a correct model of computation named refined communicating system (RCS), which is an extension of communicating automata systems with refinements. We prove that RCS only produce valid refined traces. We show how to generate RCS from mainstream protocol specification formats, such as refined multiparty session types (RMPST) or refined choreography automata. Third, we illustrate the flexibility of the framework by developing both a static analysis technique and an improved model of computation for dynamic refinement evaluation. Finally, we provide a Rust toolchain for decentralised RMPST, evaluate our implementation with a set of benchmarks from the literature, and observe that refinement overhead is negligible.

==> org_abstract.tex <==
%% Context
%
%% Issue
%Traditionally, MPST distinguish labels and payloads in the messages exchanged,
%and using different labels introduces a notion of \emph{choice} in the protocol.
%However, standard MPST does not offer the possibility to constraint the protocol
%based on the values carried in the payload of messages. To tackle this issue,
%\emph{refinements} were previously introduced to MPST, using the refined
%type-system of \(\text{F}^\star\). %
%
%
%
%
%
%% Approach
%This paper continues this preliminary study of Refined MPST by formalising the
%notion of Refined MPST and providing a generic framework to build such
%type-systems. %
%% Result
%The first and main part of this paper consists in providing a general notion of
%\emph{being well-refined} for a communicating system. Using this notion and the
%framework we developed around it, we provide an example of a refined concurrent
%system, in which refinements are dynamically checked.
%
%





Multiparty session types (MPST) is a family of type-systems for message-passing
concurrent systems which ensures\todo{"enforces"?} a set of processes behave correctly with
respect to a protocol. MPST characterise protocols by describing their sequence of
actions (sending or receiving messages). Those actions 
include selecting one message among multiple possibilities, introducing choices
in protocols. While the protocol description can specify different
possibilities for a choice, MPST do not allow to constraint the outcome based
on the value of previous messages.
\emph{Refined} multiparty session types (RMPST) extends MPST in order to constrain
communications with conditions on the values exchanged, addressing
this issue.

The first contribution of this paper is a definition
of refined session types and their semantics, in the form of newly introduced
\emph{refined communicating automata}. We provide a modular theoretical framework
to relate refined MPST to such refined communicating automata. Finally we define a
notion of \emph{correctness} for the refinements as being equivalent to the
existence of a global store of variables.

The second contribution of this paper is an implementation of the
aforementioned framework as a Rust library. We evaluate our library with a set
of micro benchmarks adapted from the litterature. We find out that the
refinement overhead is most often statistically insignificant, and minimal when
significant.


